Human Detection and Segmentation via Multi-view Consensus

Self-supervised detection and segmentation of foreground objects aims for accuracy without annotated training data. However, existing approaches predominantly rely on restrictive assumptions on appearance and motion. For scenes with dynamic activities and camera motion, we propose a multi-camera framework in which geometric constraints are embedded in the form of multi-view consistency during training via coarse 3D localization in a voxel grid and fine-grained offset regression. In this manner, we learn a joint distribution of proposals over multiple views. At inference time, our method operates on single RGB images. We outperform state-of-the-art techniques both on images that visually depart from those of standard benchmarks and on those of the classical Human3.6M dataset.

==> figures/supp_h36m_qualitative.tex <==
\begin{figure*}[hbt!]
  \centering
  {
  	\resizebox{\linewidth}{!}{
\renewcommand{\arraystretch}{0.4}
  \begin{tabular}{@{}ccccccc@{}}
   \includegraphics[width=0.137\linewidth]{figures/single_bbox_trial_4_cam_1_frame_569.jpg}
   \includegraphics[width=0.137\linewidth]{figures/single_hard_30_trial_4_cam_1_frame_569.png}&
   
      \includegraphics[width=0.137\linewidth]{figures/nsd_bbox_trial_4_cam_1_frame_569.jpg} 
   \includegraphics[width=0.137\linewidth]{figures/nsd_hard_100_trial_4_cam_1_frame_569.png} &
   
   
      \includegraphics[width=0.137\linewidth]{figures/ours_bbox_trial_4_cam_1_frame_569.jpg} 
   \includegraphics[width=0.137\linewidth]{figures/ours_hard_50_trial_4_cam_1_frame_569.png} &
   
   
   \includegraphics[width=0.137\linewidth]{figures/gt_trial_4_cam_1_frame_569.png} \\ 
   
   
   
   \includegraphics[width=0.137\linewidth]{figures/single_bbox_trial_7_cam_3_frame_1063.jpg}
   \includegraphics[width=0.137\linewidth]{figures/single_hard_30_trial_7_cam_3_frame_1063.png}&
   
   \includegraphics[width=0.137\linewidth]{figures/nsd_bbox_trial_7_cam_3_frame_1063.jpg} 
   \includegraphics[width=0.137\linewidth]{figures/nsd_hard_100_trial_7_cam_3_frame_1063.png} &
   
   
   \includegraphics[width=0.137\linewidth]{figures/ours_bbox_trial_7_cam_3_frame_1063.jpg} 
   \includegraphics[width=0.137\linewidth]{figures/ours_hard_30_trial_7_cam_3_frame_1063.png} &
   
   
   \includegraphics[width=0.137\linewidth]{figures/gt2_trial_7_cam_3_frame_1063.png} \\ 
   
   
   
   
  


 \includegraphics[width=0.137\linewidth]{figures/single_bbox_trial_0_cam_3_frame_3575.jpg}
\includegraphics[width=0.137\linewidth]{figures/single_hard_20_trial_0_cam_3_frame_3575.png}&

\includegraphics[width=0.137\linewidth]{figures/nsd_bbox_trial_0_cam_3_frame_3575.jpg} 
\includegraphics[width=0.137\linewidth]{figures/nsd_hard_100_trial_0_cam_3_frame_3575.png} &


\includegraphics[width=0.137\linewidth]{figures/ours_bbox_trial_0_cam_3_frame_3575.jpg} 
\includegraphics[width=0.137\linewidth]{figures/ours_hard_20_trial_0_cam_3_frame_3575.png} &


\includegraphics[width=0.137\linewidth]{figures/gt_trial_0_cam_3_frame_3575.png} \\ 



\includegraphics[width=0.137\linewidth]{figures/single_bbox_trial_0_cam_2_frame_2000.jpg}
\includegraphics[width=0.137\linewidth]{figures/single_hard_40_trial_0_cam_2_frame_2000.png} &

\includegraphics[width=0.137\linewidth]{figures/nsd_bbox_trial_0_cam_2_frame_2000.jpg}
\includegraphics[width=0.137\linewidth]{figures/nsd_hard_100_trial_0_cam_2_frame_2000.png}&

\includegraphics[width=0.137\linewidth]{figures/ours_bbox_trial_0_cam_2_frame_2000.jpg}
\includegraphics[width=0.137\linewidth]{figures/ours_hard_20_trial_0_cam_2_frame_2000.png}&

\includegraphics[width=0.137\linewidth]{figures/gt_trial_0_cam_2_frame_2000.png} \\




\includegraphics[width=0.137\linewidth]{figures/single_bbox_trial_9_cam_3_frame_645.jpg}
\includegraphics[width=0.137\linewidth]{figures/single_hard_20_trial_9_cam_3_frame_645.png} &

\includegraphics[width=0.137\linewidth]{figures/nsd_bbox_trial_9_cam_3_frame_645.jpg}
\includegraphics[width=0.137\linewidth]{figures/nsd_hard_100_trial_9_cam_3_frame_645.png}&

\includegraphics[width=0.137\linewidth]{figures/ours_bbox_trial_9_cam_3_frame_645.jpg}
\includegraphics[width=0.137\linewidth]{figures/ours_hard_50_trial_9_cam_3_frame_645.png}&

\includegraphics[width=0.137\linewidth]{figures/gt2_trial_9_cam_3_frame_645.png} \\



\includegraphics[width=0.137\linewidth]{figures/single_bbox_trial_6_cam_3_frame_2752.jpg}
\includegraphics[width=0.137\linewidth]{figures/single_hard_40_trial_6_cam_3_frame_2752.png} &

\includegraphics[width=0.137\linewidth]{figures/nsd_bbox_trial_6_cam_3_frame_2752.jpg}
\includegraphics[width=0.137\linewidth]{figures/nsd_hard_100_trial_6_cam_3_frame_2752.png}&

\includegraphics[width=0.137\linewidth]{figures/ours_bbox_trial_6_cam_3_frame_2752.jpg}
\includegraphics[width=0.137\linewidth]{figures/ours_hard_25_trial_6_cam_3_frame_2752.png}&

\includegraphics[width=0.137\linewidth]{figures/gt2_trial_6_cam_3_frame_2752.png} \\


\includegraphics[width=0.137\linewidth]{figures/single_bbox_trial_10_cam_3_frame_3220.jpg}
\includegraphics[width=0.137\linewidth]{figures/single_hard_20_trial_10_cam_3_frame_3220.png} &

\includegraphics[width=0.137\linewidth]{figures/nsd_bbox_trial_10_cam_3_frame_3220.jpg}
\includegraphics[width=0.137\linewidth]{figures/nsd_hard_150_trial_10_cam_3_frame_3220.png}&

\includegraphics[width=0.137\linewidth]{figures/ours_bbox_trial_10_cam_3_frame_3220.jpg}
\includegraphics[width=0.137\linewidth]{figures/ours_hard_10_trial_10_cam_3_frame_3220.png}&

\includegraphics[width=0.137\linewidth]{figures/gt2_trial_10_cam_3_frame_3225.png} \\


\includegraphics[width=0.137\linewidth]{figures/single_bbox_trial_8_cam_3_frame_1212.jpg}
\includegraphics[width=0.137\linewidth]{figures/single_hard_10_trial_8_cam_3_frame_1212.png} &

\includegraphics[width=0.137\linewidth]{figures/nsd_bbox_trial_8_cam_3_frame_1212.jpg}
\includegraphics[width=0.137\linewidth]{figures/nsd_hard_150_trial_8_cam_3_frame_1212.png}&

\includegraphics[width=0.137\linewidth]{figures/ours_bbox_trial_8_cam_3_frame_1212.jpg}
\includegraphics[width=0.137\linewidth]{figures/ours_hard_10_trial_8_cam_3_frame_1212.png}&

\includegraphics[width=0.137\linewidth]{figures/gt_trial_8_cam_3_frame_1212.png} \\


\includegraphics[width=0.137\linewidth]{figures/single_bbox_trial_8_cam_0_frame_897.jpg}
\includegraphics[width=0.137\linewidth]{figures/single_hard_10_trial_8_cam_0_frame_897.png} &

\includegraphics[width=0.137\linewidth]{figures/nsd_bbox_trial_8_cam_0_frame_897.jpg}
\includegraphics[width=0.137\linewidth]{figures/nsd_hard_2_trial_8_cam_0_frame_897.png}&

\includegraphics[width=0.137\linewidth]{figures/ours_bbox_trial_8_cam_0_frame_897.jpg}
\includegraphics[width=0.137\linewidth]{figures/ours_hard_50_trial_8_cam_0_frame_897.png}&

\includegraphics[width=0.137\linewidth]{figures/gt2_trial_8_cam_0_frame_897.png} \\ 

 
 
   
    \includegraphics[width=0.137\linewidth]{figures/single_bbox_trial_25_cam_2_frame_3150.jpg}
   \includegraphics[width=0.137\linewidth]{figures/single_hard_3_trial_25_cam_2_frame_3150.png}&
   
   \includegraphics[width=0.137\linewidth]{figures/nsd_bbox_trial_25_cam_2_frame_3150.jpg} 
   \includegraphics[width=0.137\linewidth]{figures/nsd_hard_3_trial_25_cam_2_frame_3150.png} &
   
   
   \includegraphics[width=0.137\linewidth]{figures/ours_bbox_trial_25_cam_2_frame_3150.jpg} 
   \includegraphics[width=0.137\linewidth]{figures/ours_hard_3_trial_25_cam_2_frame_3150.png} &
   
   
   \includegraphics[width=0.137\linewidth]{figures/gt_trial_25_cam_2_frame_3150.png} \\ 


 \\




{\fontsize{10}{5}\selectfont  (a)~Katircioglu et al.~\cite{Katircioglu20}}& {\fontsize{10}{5}\selectfont(b) Rhodin et al.~\cite{Rhodin19a}} &  {\fontsize{10}{5}\selectfont (c) Ours}  & {\fontsize{10}{5}\selectfont (d) GT }  \\ \\
  \end{tabular}}
}
  \caption{\textbf{Qualitative results on the {\human} dataset.} (a) The detection and segmentation mask results of Katircioglu et al.~\cite{Katircioglu20} trained and tested on single images. (b) The results of~\cite{Rhodin19a} trained with a pair of camera views and tested on single images. (c) Our predictions obtained from the model trained with the 4-cam multi-view consistency and tested on single images. (d) Ground truth.}
  \label{fig:supp_h36m_qual}
\end{figure*}

==> figures/supp_handheld_qualitative.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[hbt!]
  \centering
  {
  	\resizebox{\linewidth}{!}{
\renewcommand{\arraystretch}{0.4}
  \begin{tabular}{@{}ccccc@{}}
   \includegraphics[width=0.45\linewidth]{figures/scam_bbox_trial_8_cam_5_frame_16974.jpg}
   \includegraphics[width=0.45\linewidth]{figures/scam_hard_trial_8_cam_5_frame_16974.jpg}&
   
      \includegraphics[width=0.45\linewidth]{figures/mcam_bbox_trial_9_cam_5_frame_16974.jpg} 
   \includegraphics[width=0.45\linewidth]{figures/mcam_hard_trial_9_cam_5_frame_16974.jpg} &
   
   \includegraphics[width=0.45\linewidth]{figures/gt_frame_016974.jpg} \\ 
   
   
   
    \includegraphics[width=0.45\linewidth]{figures/scam_bbox_trial_8_cam_5_frame_19061.jpg}
   \includegraphics[width=0.45\linewidth]{figures/scam_trial_8_cam_5_frame_19061.jpg}&
   
   \includegraphics[width=0.45\linewidth]{figures/mcam_bbox_trial_9_cam_5_frame_19061.jpg} 
   \includegraphics[width=0.45\linewidth]{figures/mcam_hard_trial_9_cam_5_frame_19061.jpg} &
   
   \includegraphics[width=0.45\linewidth]{figures/gt_frame_019061.jpg} \\ 
   
   
    \includegraphics[width=0.45\linewidth]{figures/scam_bbox_trial_8_cam_5_frame_7368.jpg}
   \includegraphics[width=0.45\linewidth]{figures/scam_hard_trial_8_cam_5_frame_7368.jpg}&
   
   \includegraphics[width=0.45\linewidth]{figures/mcam_bbox_trial_9_cam_5_frame_7368.jpg} 
   \includegraphics[width=0.45\linewidth]{figures/mcam_hard_trial_9_cam_5_frame_7368.jpg} &
   
   \includegraphics[width=0.45\linewidth]{figures/gt_frame_007368.jpg} \\ 
   
   
    \includegraphics[width=0.45\linewidth]{figures/scam_bbox_trial_8_cam_5_frame_4276.jpg}
   \includegraphics[width=0.45\linewidth]{figures/scam_hard_trial_8_cam_5_frame_4276.jpg}&
   
   \includegraphics[width=0.45\linewidth]{figures/mcam_bbox_trial_9_cam_5_frame_4276.jpg} 
   \includegraphics[width=0.45\linewidth]{figures/mcam_hard_trial_9_cam_5_frame_4276.jpg} &
   
   \includegraphics[width=0.45\linewidth]{figures/gt_frame_004276.jpg} \\ 
   
   
    \includegraphics[width=0.45\linewidth]{figures/scam_bbox_trial_8_cam_4_frame_10779.jpg}
   \includegraphics[width=0.45\linewidth]{figures/scam_hard_trial_8_cam_4_frame_10779.jpg}&
   
   \includegraphics[width=0.45\linewidth]{figures/mcam_bbox_trial_9_cam_4_frame_10779.jpg} 
   \includegraphics[width=0.45\linewidth]{figures/mcam_hard_trial_9_cam_4_frame_10779.jpg} &
   
   \includegraphics[width=0.45\linewidth]{figures/gt_frame_010779.jpg} \\ 
   
    \includegraphics[width=0.45\linewidth]{figures/scam_bbox_trial_8_cam_4_frame_13224.jpg}
   \includegraphics[width=0.45\linewidth]{figures/scam_hard_trial_8_cam_4_frame_13224.jpg}&
   
   \includegraphics[width=0.45\linewidth]{figures/mcam_bbox_trial_9_cam_4_frame_13224.jpg} 
   \includegraphics[width=0.45\linewidth]{figures/mcam_hard_trial_9_cam_4_frame_13224.jpg} &
   
   \includegraphics[width=0.45\linewidth]{figures/gt_frame_013224.jpg} \\ 
   
    \includegraphics[width=0.45\linewidth]{figures/scam_bbox_trial_8_cam_4_frame_8921.jpg}
   \includegraphics[width=0.45\linewidth]{figures/scam_hard_trial_8_cam_4_frame_8921.jpg}&
   
   \includegraphics[width=0.45\linewidth]{figures/mcam_bbox_trial_9_cam_4_frame_8921.jpg} 
   \includegraphics[width=0.45\linewidth]{figures/mcam_hard_trial_9_cam_4_frame_8921.jpg} &
   
   \includegraphics[width=0.45\linewidth]{figures/gt_frame_008921.jpg} \\ 
   
    \includegraphics[width=0.45\linewidth]{figures/scam_bbox_trial_8_cam_4_frame_1111.jpg}
   \includegraphics[width=0.45\linewidth]{figures/scam_hard_trial_8_cam_4_frame_1111.jpg}&
   
   \includegraphics[width=0.45\linewidth]{figures/mcam_bbox_trial_9_cam_4_frame_1111.jpg} 
   \includegraphics[width=0.45\linewidth]{figures/mcam_hard_trial_9_cam_4_frame_1111.jpg} &
   
   \includegraphics[width=0.45\linewidth]{figures/gt_frame_001111.jpg} \\ 
   
   
     \includegraphics[width=0.45\linewidth]{figures/scam_bbox_trial_8_cam_3_frame_400.jpg}
   \includegraphics[width=0.45\linewidth]{figures/scam_hard_trial_8_cam_3_frame_400.jpg}&
   
   \includegraphics[width=0.45\linewidth]{figures/mcam_bbox_trial_9_cam_3_frame_400.jpg} 
   \includegraphics[width=0.45\linewidth]{figures/mcam_hard_trial_9_cam_3_frame_400.jpg} &
   
   \includegraphics[width=0.45\linewidth]{figures/gt_frame_000400.jpg} \\ 
   
   
    \includegraphics[width=0.45\linewidth]{figures/scam_bbox_trial_8_cam_3_frame_8063.jpg}
   \includegraphics[width=0.45\linewidth]{figures/scam_trial_8_cam_3_frame_8063.jpg}&
   
   \includegraphics[width=0.45\linewidth]{figures/mcam_bbox_trial_9_cam_3_frame_8063.jpg} 
   \includegraphics[width=0.45\linewidth]{figures/mcam_hard_trial_9_cam_3_frame_8063.jpg} &
   
   \includegraphics[width=0.45\linewidth]{figures/gt_frame_008063.jpg} \\ 
   
   
    \includegraphics[width=0.45\linewidth]{figures/scam_bbox_trial_8_cam_3_frame_2750.jpg}
   \includegraphics[width=0.45\linewidth]{figures/scam_hard_trial_8_cam_3_frame_2750.jpg}&
   
   \includegraphics[width=0.45\linewidth]{figures/mcam_bbox_trial_9_cam_3_frame_2750.jpg} 
   \includegraphics[width=0.45\linewidth]{figures/mcam_hard_trial_9_cam_3_frame_2750.jpg} &
   
   \includegraphics[width=0.45\linewidth]{figures/gt_frame_002750.jpg} \\ \\ \\



{ \fontsize{22}{5}\selectfont  (a)~Katircioglu et al.~\cite{Katircioglu20}} &  {\fontsize{22}{5}\selectfont  (b) Ours}  & {\fontsize{22}{5}\selectfont  (c) GT }  \\ 
  \end{tabular}}
}

  \caption{\textbf{Qualitative results on the {\handheld{}} dataset.} (a) The detection and segmentation mask results of~\cite{Katircioglu20} trained and tested on single images. (b) The predictions of our model trained using 3-camera multi-view consistency and tested on single images. (c) Ground truth. Our results are generally more accurate, which justifies the effort invested in calibrating the cameras.}
  \label{fig:supp_handheld_qual}
\end{figure*}


==> figures/supp_ski_qualitative.tex <==
\begin{figure*}[hbt!]
  \centering
  {
\renewcommand{\arraystretch}{0.4}
  \begin{tabular}{@{}cccccc@{}}
  
   
   \includegraphics[width=0.16\linewidth]{figures/bbox_trial_412_cam_3_frame_110.jpg} &\hspace{-4.0mm}
   \includegraphics[width=0.16\linewidth]{figures/umod_412_cam3_110.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/arp_412_cam3_110.png} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/single_trial_412_cam_3_frame_110.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/mcam_ours_trial_412_cam_3_frame_110.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/gt_412_cam3_frame_000110.jpg} \\
   
   
    \includegraphics[width=0.16\linewidth]{figures/bbox_trial_405_cam_6_frame_170.jpg} &\hspace{-4.0mm}
   \includegraphics[width=0.16\linewidth]{figures/umod_405_cam6_170.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/arp_405_cam6_170.png} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/single_trial_405_cam_6_frame_170.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/mcam_ours_trial_405_cam_6_frame_170.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/gt_405_cam6_frame_000170.jpg} \\
   
   
   
   \includegraphics[width=0.16\linewidth]{figures/bbox_trial_412_cam_1_frame_191.jpg} &\hspace{-4.0mm}
   \includegraphics[width=0.16\linewidth]{figures/umod_412_cam1_191.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/arp_412_cam1_191.png} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/single_trial_412_cam_1_frame_191.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/mcam_ours_trial_412_cam_1_frame_191.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/gt_412_cam1_frame_000191.jpg} \\
   
   
    \includegraphics[width=0.16\linewidth]{figures/bbox_trial_405_cam_2_frame_194.jpg} &\hspace{-4.0mm}
   \includegraphics[width=0.16\linewidth]{figures/umod_405_cam2_194.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/arp_405_cam2_194.png} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/single_trial_405_cam_2_frame_194.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/mcam_ours_trial_405_cam_2_frame_194.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/gt_405_cam2_194_frame_000194.jpg} \\
   
   
   \includegraphics[width=0.16\linewidth]{figures/bbox_trial_412_cam_1_frame_178.jpg} &\hspace{-4.0mm}
   \includegraphics[width=0.16\linewidth]{figures/umod_412_cam1_178.jpg} &\hspace{-4mm}
      \includegraphics[width=0.16\linewidth]{figures/arp_412_cam1_178.png} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/single_trial_412_cam_1_frame_178.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/ours_trial_412_cam_1_frame_178.jpg} &\hspace{-4mm}
   \includegraphics[width=0.16\linewidth]{figures/gt_412_cam1_frame_000178.jpg} \\ 
   
   
  \includegraphics[width=0.16\linewidth]{figures/bbox_trial_405_cam_5_frame_200.jpg} &\hspace{-4.0mm}
  \includegraphics[width=0.16\linewidth]{figures/umod_405_cam5_200.jpg}& \hspace{-4mm}
     \includegraphics[width=0.16\linewidth]{figures/arp_405_cam5_200.png}& \hspace{-4mm}
  \includegraphics[width=0.16\linewidth]{figures/single_trial_405_cam_5_frame_200.jpg}& \hspace{-4mm}
    \includegraphics[width=0.16\linewidth]{figures/mcam_ours_trial_405_cam_5_frame_200.jpg}& \hspace{-4mm}
  \includegraphics[width=0.16\linewidth]{figures/gt_405_cam5_frame_000200.jpg}  \\
  
  \includegraphics[width=0.16\linewidth]{figures/bbox_trial_405_cam_1_frame_100.jpg} &\hspace{-4.0mm}
  \includegraphics[width=0.16\linewidth]{figures/unsup_mov_405_cam1_100.jpg}& \hspace{-4mm}
  \includegraphics[width=0.16\linewidth]{figures/arp_trial_405_cam1_frame_100.png}& \hspace{-4mm}
  \includegraphics[width=0.16\linewidth]{figures/pred_405_cam1_100.png}& \hspace{-4mm}
    \includegraphics[width=0.16\linewidth]{figures/mcam_ours_trial_405_cam_1_frame_000100.jpg}& \hspace{-4mm}
  \includegraphics[width=0.16\linewidth]{figures/gt_405_cam1_100.png}  \\
  
%\includegraphics[width=0.15\linewidth]{figures/confidence_trial_405_cam_4_frame_135.jpg} &
%\includegraphics[width=0.15\linewidth]{figures/pred_405_cam4_135.png}& \hspace{-8mm}
%\includegraphics[width=0.15\linewidth]{figures/unsup_dilate_405_cam4_135.png}& \hspace{-12mm}
%\includegraphics[width=0.15\linewidth]{figures/gt_405_cam4_135.png}  \\
%\includegraphics[width=0.15\linewidth]{figures/confidence_trial_405_cam_2_frame_194.jpg}&
%\includegraphics[width=0.15\linewidth]{figures/pred_405_cam2_194.png} &\hspace{-8mm}
%\includegraphics[width=0.15\linewidth]{figures/unsup_dilate_405_cam2_194.png}& \hspace{-12mm}
%\includegraphics[width=0.15\linewidth]{figures/gt_405_cam2_194.png}\\

%\includegraphics[width=0.16\linewidth]{figures/bbox_trial_412_cam_5_frame_84.jpg} &\hspace{-4.0mm}
%\includegraphics[width=0.16\linewidth]{figures/unsup_dilate_412_cam5_84.png} &\hspace{-4mm}
%\includegraphics[width=0.16\linewidth]{figures/unsup_mov_412_cam5_84.jpg} &\hspace{-4mm}
%\includegraphics[width=0.16\linewidth]{figures/arp_412_cam5_84.png} &\hspace{-4mm}
%\includegraphics[width=0.16\linewidth]{figures/pred_412_cam5_84.jpg} &\hspace{-4mm}
%\includegraphics[width=0.16\linewidth]{figures/gt_412_cam5_84.jpg} \\

%\includegraphics[width=0.16\linewidth]{figures/confidence_trial_412_cam_6_frame_185.jpg} &\hspace{-4.0mm}
%\includegraphics[width=0.16\linewidth]{figures/unsup_dilate_412_cam6_185.png} &\hspace{-4mm}
%\includegraphics[width=0.16\linewidth]{figures/unsup_mov_412_cam6_185.jpg} &\hspace{-4mm}
%\includegraphics[width=0.16\linewidth]{figures/pred_412_cam6_185.png} &\hspace{-4mm}
%\includegraphics[width=0.16\linewidth]{figures/gt_412_cam6_185.png} \\

%\includegraphics[width=0.16\linewidth]{figures/confidence_trial_405_cam_1_frame_175.jpg} &\hspace{-4.0mm}
%\includegraphics[width=0.16\linewidth]{figures/unsup_dilate_405_cam1_175.png} &\hspace{-4mm}
%\includegraphics[width=0.16\linewidth]{figures/unsup_mov_405_cam1_175.jpg} &\hspace{-4mm}
%\includegraphics[width=0.16\linewidth]{figures/arp_405_cam1_175.png} &\hspace{-4mm}
%\includegraphics[width=0.16\linewidth]{figures/pred_405_cam1_175.png} &\hspace{-4mm}
%\includegraphics[width=0.16\linewidth]{figures/gt_405_cam1_175.png} \\

\includegraphics[width=0.16\linewidth]{figures/bbox_trial_412_cam_6_frame_181.jpg} &\hspace{-4.0mm}
\includegraphics[width=0.16\linewidth]{figures/umod_412_cam6_181.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/arp_412_cam6_181.png} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/single_trial_412_cam_6_frame_181.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/mcam_ours_trial_412_cam_6_frame_181.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/gt_412_cam6_frame_000181.jpg} \\ 

\includegraphics[width=0.16\linewidth]{figures/bbox_trial_405_cam_1_frame_212.jpg} &\hspace{-4.0mm}
\includegraphics[width=0.16\linewidth]{figures/umod_405_cam1_212.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/arp_405_cam1_212.png} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/single_trial_405_cam_1_frame_212.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/mcam_ours_trial_405_cam_1_frame_212.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/gt_405_cam1_frame_000212.jpg} \\

%\includegraphics[width=0.15\linewidth]{figures/confidence_trial_405_cam_5_frame_200.jpg} &\hspace{2.2mm}
%\includegraphics[width=0.15\linewidth]{figures/pred_405_cam5_200.png} &\hspace{-1mm}
%\includegraphics[width=0.15\linewidth]{figures/unsup_dilate_405_cam5_200.png} &\hspace{-4mm}
%\includegraphics[width=0.15\linewidth]{figures/gt_405_cam5_200.png} \\

%\includegraphics[width=0.15\linewidth]{figures/confidence_trial_412_cam_4_frame_120.jpg} &
%\includegraphics[width=0.15\linewidth]{figures/pred_412_cam4_120.png} &\hspace{-8mm}
%\includegraphics[width=0.15\linewidth]{figures/unsup_dilate_412_cam4_120.png} &\hspace{-12mm}
%\includegraphics[width=0.15\linewidth]{figures/gt_412_cam4_120.png} \\

\includegraphics[width=0.16\linewidth]{figures/bbox_trial_405_cam_4_frame_142.jpg} &\hspace{-4.0mm}
\includegraphics[width=0.16\linewidth]{figures/umod_405_cam4_142.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/arp_405_cam4_142.png} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/single_trial_405_cam_4_frame_142.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/mcam_ours_trial_405_cam_4_frame_142.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/gt_405_cam4_frame_000142.jpg} \\ 


\includegraphics[width=0.16\linewidth]{figures/bbox_trial_405_cam_3_frame_190.jpg} &\hspace{-4.0mm}
\includegraphics[width=0.16\linewidth]{figures/umod_405_cam3_190.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/arp_405_cam3_190.png} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/single_trial_405_cam_3_frame_190.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/mcam_ours_trial_405_cam_3_frame_190.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/gt_405_cam3_frame_000190.jpg} \\  


\includegraphics[width=0.16\linewidth]{figures/bbox_trial_405_cam_6_frame_115.jpg} &\hspace{-4.0mm}
\includegraphics[width=0.16\linewidth]{figures/umod_405_cam6_115.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/arp_405_cam6_115.png} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/single_trial_405_cam_6_frame_115.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/mcam_ours_trial_405_cam_6_frame_115.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/gt_405_cam6_frame_000115.jpg} \\ 


\includegraphics[width=0.16\linewidth]{figures/bbox_trial_405_cam_3_frame_86.jpg} &\hspace{-4.0mm}
\includegraphics[width=0.16\linewidth]{figures/unsup_mov_405_cam3_86.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/arp_405_cam3_86.png} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/pred_405_cam3_86.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/mcam_ours_trial_405_cam_3_frame_000086.jpg} &\hspace{-4mm}
\includegraphics[width=0.16\linewidth]{figures/gt_405_cam3_86.jpg}   \\

\\

  
  {\fontsize{8}{5}\selectfont  \hspace{-1mm}(a) Input/Ours detection}& \hspace{-1mm} {\fontsize{8}{5}\selectfont (b) Yang et al.~\cite{Yang19c}}&\hspace{-4mm} {\fontsize{8}{5}\selectfont (c) Koh et al.~\cite{Koh17b}} &\hspace{-4mm} {\fontsize{8}{5}\selectfont (d) Katircioglu et al.~\cite{Katircioglu20}}&\hspace{-4mm}   {\fontsize{8}{5}\selectfont (e) Ours}  &\hspace{-4mm}  {\fontsize{8}{5}\selectfont (f) GT }  \\ \\
  \end{tabular}}

  \caption{ \textbf{Qualitative results on the \ski{}.} (a) Input images with our predicted bounding box overlaid in red. (b) Segmentation mask prediction of~\cite{Yang19c}. (c) Segmentation mask prediction of~\cite{Koh17b}. (d) Segmentation mask prediction of~\cite{Katircioglu20} (e) Our segmentation mask prediction. (f) Ground truth segmentation mask. Note that, unlike our method,~\cite{Koh17b} and~\cite{Yang19c} use explicit temporal cues at inference time.}
  \label{fig:supp_ski_qual}
\end{figure*}
